Exoplanet Detection via Differentiable Rendering

Direct imaging of exoplanets is crucial for advancing our understanding of planetary systems beyond our solar system, but it faces significant challenges due to the high contrast between host stars and their planets. Wavefront aberrations introduce speckles in the telescope science images, which are patterns of diffracted starlight that can mimic the appearance of planets, complicating the detection of faint exoplanet signals. Traditional post-processing methods, operating primarily in the image intensity domain, do not integrate wavefront sensing data. These data, measured mainly for adaptive optics corrections, have been overlooked as a potential resource for post-processing, partly due to the challenge of the evolving nature of wavefront aberrations. In this paper, we present a differentiable rendering approach that leverages these wavefront sensing data to improve exoplanet detection. Our differentiable renderer models wave-based light propagation through a coronagraphic telescope system, allowing gradient-based optimization to significantly improve starlight subtraction and increase sensitivity to faint exoplanets. Simulation experiments based on the James Webb Space Telescope configuration demonstrate the effectiveness of our approach, achieving substantial improvements in contrast and planet detection limits. Our results showcase how the computational advancements enabled by differentiable rendering can revitalize previously underexploited wavefront data, opening new avenues for enhancing exoplanet imaging and characterization.

==> sections/1_introduction.tex <==



\iffalse
Direct-imaging is a vital method for detection and characterization of exoplanets, complementing indirect methods like transit and radial velocity by being sensitive to companions in different regions of parameter space (e.g. planets at more than 10 AU of separation from the star). The development of NASA space missions like the current James Webb Space Telescope (JWST), and in the future the Roman Space Telescope and the Habitable Worlds Observatory, as well as other ground-based instruments like the Gemini Planet Imager 2.0 and the Extremely Large Telescope, mark a decisively important period in the study of exoplanets by direct-imaging, with the prospect of imaging Earth-like planets and finding life in other worlds.


The main challenge for exoplanet imaging is the very high level of \textbf{contrast} needed to detect a planet; that is, the ability to identify point-sources orders of magnitude fainter than the host star next to them. This problem is especially challenging given that light suffers several kinds of wavefront errors that translate into \textbf{speckles} in the science detector, producing fake signals very similar to that of a planet. The dependence of the speckles on the wavefront errors is also a complicated one, since the optical systems (coronagraphs) designed to suppress starlight to make the planet more visible consist of several masks both at the pupil and focal planes (see Figure \ref{fig:coronagraph}).

Additionally, while some of the wavefront errors are fast-varying and therefore can be roughly averaged out with sufficiently long exposures (such as those from atmospheric turbulence in ground-based telescopes), other wavefront errors are slow-varying, causing static or quasi-static speckle patterns, which hardly average out over very long exposures. Furthermore, some wavefront errors are measured by wavefront sensing systems (for example, to partially correct for them using adaptive optics in ground-based instruments, see Figure \ref{fig:groundbased}), but other types of wavefront errors are not measured, such as those arising from instrument defects after the wavefront sensor (called Non-Common Path Aberrations, or NCPAs). This complex interaction of several types of wavefront errors that result in complicated and undesired speckles that drown the planet signal, is the fundamental challenge for high-contrast exoplanet imaging.

The next sections provide an overview of coronagraphy and wavefront error contributions to the final images.
\fi

==> sections/2_coronography.tex <==

\section{Coronagraphy}
\label{sec:corona}

Coronagraphy refers to the use of hardware to suppress starlight as much as possible, allowing for the light of the planet to be more easily detectable. The exact design of each coronagraphic instrument will vary from case to case (JWST alone has several available coronagraphs, for example). Figure \ref{fig:coronagraph} shows a diagram of the coronagraph instrument used in GPI. Common general elements to be found in a coronagraph include (following the left-to-right order in the bottom half of the figure):

\begin{itemize}
    \item \textbf{Pupil aperture:} Actual entrance of light into the telescope. 
    \item \textbf{Apodizer:} Smooths the edges of the entrance pupil to mitigate diffraction patterns. Operates in the pupil plane.
    \item \textbf{Focal plane mask:} Effectively blocks central region of the image, where the star is located. Operates in the image plane In a simple case, a simple circular mask performs the blocking. Slightly different mechanisms to perform the same task can also be used.
    \item \textbf{Lyot Stop:} Mask to further suppress remaining diffraction patterns. Operates in the pupil plane.
    \item \textbf{Detector:} Where the final image is formed.
\end{itemize}

Each element prior to the detector essentially corresponds to a transmission function for the incoming electric field (evidently, masks in the image plane are carried out as transmission functions in the Fourier domain). The specific design (e.g. the dimensions of the focal plane mask or whether or not the instrument has an apodizer at all) vary from instrument to instrument.

To a good approximation in the case of exoplanet imaging, two Point-Spread Functions (PSFs) are involved in the image formation process. The first PSF corresponds to the central PSF of the star (see right-most panel in the bottom half of Figure \ref{fig:coronagraph}) which will be affected by the central focal plane mask. Since the star is much brighter than the planets, even after the occulting masks the remaining starlight will dominate in intensity and will present speckle patterns from wavefront errors (see Section \ref{sec:wfe}).

The second PSF corresponds to point sources outside the central region of the image (e.g. planets), and therefore is not affected by the focal plane mask. To a good approximation, the PSF will be spatially invariant for point-sources in this region of the image.


==> sections/3_wfe.tex <==

\section{Wavefront error sources}
\label{sec:wfe}

The obstacles for exoplanet imaging in ground-based instruments and in space-based instruments share many similarities in terms of sources of wavefront errors. See Figures \ref{fig:groundbased} and \ref{fig:spacebased} for a schematic of each. The sections below summarize each one, and highlight their differences.

For reference, observation sequences are very similar for ground-based instruments and space-based instruments, except for exposure time. A typical single observing sequence with a coronagraphic instrument on the ground (e.g. GPI) lasts around one hour, during which 40 to 60 total images are collected, where each image consists of an integration of around 60 seconds. For space telescopes like JWST, due to higher wavefront stability, longer exposure times are possible, around the order of 10 minutes of integration for a single image. 

Also, the Integral Field Spectrograph (IFS) in GPI can take simultaneous measurements in 37 wavelengths, and the NIRCam instrument in JWST can take simultaneous measurements in 2 wavelengths.

\subsection{Ground-based instruments}
\label{sec:wfeground}

Ground-based instruments, such as the Gemini Planet Imager, face primarily two sources of wavefront errors: atmospheric turbulence and Non-Common Path Aberrations (NCPAs). See Figure \ref{fig:groundbased}.

Light coming from the objects of interest passes through the atmosphere, which changes (i.e. suffers slight changes in the index of refraction due to temperature fluctuations) on the millisecond timescale, causing wavefront errors that also vary on the millisecond timescale. These aberrations are partially corrected by an Adaptive Optics (AO) system, following the path shown in Figure \ref{fig:groundbased}. Deformable mirrors partially correct the wavefront aberrations, then the light (with the residual aberrations) goes through a beam-splitter: on the one hand, the wavefronts enter the coronagraph pupil and propagate through the optics (see Figure \ref{fig:coronagraph}); on the other hand, the residual aberrations are sent to a wavefront sensor, which then through a control system updates the actuators in the deformable mirrors to improve the correction. Both the measurements of the wavefront sensor and the updates to the deformable mirrors occur in real time during the observation, and are carried out on the millisecond timescale, similar to the timescale of the atmosphere variations. 

The AO system wavefront corrections are never perfect, due to a variety of factors, such as the speed of the AO system (some atmospheric aberrations change faster than the AO system can correct for them), the limited degrees of freedom of the deformable mirrors (i.e. a finite number of actuators), measurement errors in the wavefront sensor, among others. For these reasons, residual aberrations caused by atmospheric turbulence end up propagating through the coronagraph and onto the science detector, causing fast-varying speckles. Due to the short timescales, with sufficiently long exposures most atmospheric wavefront error would average out to zero. As a consequence, also fast-varying speckle patterns on the science camera average out, but not to zero (since the detector measures the intensity of the electric field, that is, always a positive number), but to a sort of relatively-low-intensity "halo" across the image.

The other main source of wavefront errors are NCPAs, that is, aberrations introduced by the optical system itself that occur after the light has been measured by the wavefront sensor. These errors are effectively unknown (they are not measured by any sensor), and are caused by defects such as drifting of the optics, slow defocus-and-focus, thermal breathing of the instrument, among others. These aberrations, then, typically evolve over longer timescales, comparable to the duration of the entire observing sequence, and therefore do not cancel out over observation timescales. These aberrations result in static or quasi-static speckle patterns in the science detector, which also do not average out during observation timescales.

While direct measurements of NCPAs are not collected, some insight into their statistical properties can be gained by analyzing internal light source data. That is, science camera measurements collected when only the internal light source of the instrument is on, instead of when a real observation to an astronomical object is being done. Since the internal light source of the instrument does not traverse the atmosphere, the light that makes it to the science detector has only travelled through the optics of the instrument, so it is in principle  only subject to NCPAs. Science measurements of internal light source can, therefore, yield insights into some of the statistical properties of NCPAs.

\subsection{Space-based instruments}
\label{sec:wfespace}

Space-based instruments, such as JWST, experience similar sources of wavefront error as ground-based instruments, though with some important differences. Many important differences arise from the lack of atmosphere and the significant increase in instrument stability compared to the ground-based counterparts. See Figure \ref{fig:spacebased} for a summary and schematic depiction of these aberrations.

Since space-based instruments do not have to deal with atmospheric turbulence, they are not subject to these fast-varying wavefront aberrations. For the same reason, they typically do not have an AO system to correct for these aberrations in real time. 

Wavefront errors are still introduced before the coronagraph due to other factors, however. In the particular case of JWST, for example, misalignments of the primary mirrors cause wavefront errors. Wavefront measurements of these aberrations are carried out every two days, with corrections (realignments of the mirrors) carried out roughly every two weeks. These cadences are reasonable considering the high stability of the instrument (e.g. see Figure 2 in \url{https://jwst-docs.stsci.edu/jwst-observatory-hardware/jwst-wavefront-sensing-and-control}), so these wavefront errors can be considered slow-varying, static or quasi-static.

On the other hand, JWST also presents NCPAs due to aberrations introduced after the wavefront sensor by similar physical factors as NCPAs in ground-based instruments. Similar tests with internal light sources have been used to characterize wavefront errors in the instrument, but they are not measured during the observing sequence or close to it (unlike mirror misalignment errors).

Therefore, the main similarities between ground-based and space-based instruments regarding wavefront errors are:

\begin{itemize}
    \item Both ground-based and space-based instruments present Non-Common Path Aberrations: wavefront errors introduced after the wavefront sensor (they are, then, not directly measured), which generally change over long timescales.
    \item Both ground-based and space-based instruments carry measurements of wavefront errors before the light enters the coronagraph, though with different cadences.
\end{itemize}

The main differences are:

\begin{itemize}
    \item Space-based instruments are more stable than ground-based instruments, so measurements of wavefront errors are taken much less frequently (e.g. every two days for JWST as opposed to every millisecond with GPI).
    \item Ground-based instruments are subject to millisecond-timescale-varying wavefront errors due to atmospheric turbulence, which are partially corrected by AO systems; the residual aberrations that make it to the coronagraph are measured by the wavefront sensor. Space-based instruments are not subject to atmospheric errors and do not have AO systems for real-time correction.
\end{itemize}

==> sections/4_current_postproc.tex <==

\section{Current post-processing techniques}
\label{sec:current_post}

Most post-processing techniques routinely used to suppress speckle noise are based on stellar PSF subtraction: from a collection of reference images, use principal component analysis (PCA) to subtract the stellar PSF from the target images and help reveal the planets. 

Several methods for building the collection of images exist; for example:

\begin{itemize}
    \item \textbf{Angular Differential Imaging (ADI)} (\cite{Marois_2006}) consists in taking images of the same target (i.e. the same star) but rotating the field of view. In this way, many the speckles due to instrument aberrations would remain static or quasi-static at different rotations, but the planet signal would rotate with the rest of the field of view (since over observing sequences the planet is essentially static). This allows to better distinguish speckles from true planet signals.
    \item \textbf{Spectral Simultaneous Differential Imaging (SSDI)} (e.g. \cite{Marois2000Efficient}) consists in taking images of the same target and at the same orientation but at different wavelengths simultaneously. Since diffraction patterns are wavelength-dependent, speckle noise will move at different wavelengths, but the planet signal will not.
    \item  \textbf{Reference Star Differential Imaging (RSDI)}  (e.g. \cite{ruane2019reference}) consists in taking images of reference stars or using already existing images of such stars from archival data to build the collection of images. This is especially relevant for space-based telescopes such as JWST.
\end{itemize}

Once with a relevant collection of reference images, these images are combined to produce a reference PSF to subtract from the target images. Common algorithms to do this include LOCI (\cite{Lafreniere_2007}) and KLIP (\cite{Soummer2012Detection}). Essentially a PCA-based method is used to build a reference image, subtract it from target images, and help mitigate speckle patterns to allow better contrast sensitivity.


==> sections/5_diffsim.tex <==
\section{Enhanced Post-processing via Differentiable Simulation}
Traditional post-processing techniques aim to suppress the starlight and reveal the faint exoplanet signal, but these methods often face limitations in terms of their ability to effectively integrate and leverage the available wavefront sensing data. This limitation becomes particularly critical in scenarios with extremely low signal-to-noise ratios, where the accurate estimation and correction of wavefront errors can significantly impact the detectability of the exoplanet signal.

To address these challenges and advance the planet detection performance through the post-processing approach, we propose a novel approach based on differentiable simulation. 
By constructing a differentiable model of the image formation process in a high-contrast imaging system, we enable the inversion of the forward model to estimate previously unknown wavefront error components, allowing us to go beyond the detection limits of traditional post-processing pipelines.

The key idea behind our differentiable simulation framework is to establish a direct and differentiable connection between the wavefront error maps and the observed science images with speckles. 
This differentiable simulation framework allows us to leverage the power of gradient-based optimization techniques to refine our estimates of the true wavefront errors, thereby improving the accuracy of the reconstructed stellar point spread function (PSF) and enhancing the detectability of faint exoplanet signals.

In this section, we present the mathematical formulation of our differentiable simulator and describe its architecture, which is designed to model the propagation of light through a coronagraphic optical system. 
We demonstrate the effectiveness of our approach through a series of simulation experiments, showcasing its ability to refine wavefront error estimates, suppress speckle noise, and improve the overall performance of starlight subtraction.

\input{figures/fig_4}

\subsection{Differentiable Simulation}

Differentiable simulation and rendering of visual data have transformed various domains, including computer graphics and computational imaging, by enabling the optimization of parameters through gradient descent on a differentiable simulation's output.
This paradigm has unlocked previously intractable inverse problems in imaging and enabled efficient computations to obtain solutions.

In computer graphics, differentiable rendering has enabled the rendering of photorealistic images from parametric scene descriptions, via iterative optimizations of the rendering parameters to match target images.
Similarly, in computational imaging, differentiable simulation has revolutionized the design of optical systems by enabling the optimization of optical system parameters to achieve desired imaging characteristics. 
Our work builds upon these advancements by introducing a differentiable simulator specifically designed for the challenges of high-contrast astronomical imaging, crucial for the detection of exoplanets.

Our proposed differentiable simulator, denoted as $\mathcal{G}_{sim}$, takes the position of the central star $p_{star}$ and a wavefront error map $\phi$ as inputs, and generates a simulated science image $\hat{y}$ that approximates the actual measurements recorded by the science camera:

\begin{equation}
\hat{y} = \mathcal{G}_{sim}(p_{star}, \phi) .
\end{equation}

The simulator is designed as a composition of differentiable tensor operations modeling the propagation of light through the coronagraphic optical system. By leveraging the automatic differentiation capabilities of machine learning frameworks, $\mathcal{G}_{sim}$ enables gradient computation with respect to all input parameters. This allows the use of efficient gradient-based optimization techniques to infer the latent wavefront error maps from the observed focal plane images.

\input{figures/fig_5}

\input{figures/fig_6}

\input{figures/fig_7}

The simulator's architecture is designed with differentiability in mind, enabling the seamless integration of gradient descent optimization techniques. 
By iteratively refining the wavefront error maps based on the discrepancies between the simulated and observed focal plane images, we progressively improve our estimates of the true wavefront errors.

Let $\phi_{i}$ denote the true wavefront error map for the $i$-th observation, $y_{i}$ represent the corresponding focal plane image, and $p_{star}$ indicate the position of the central star. 
The forward physical model of the optical system can be expressed as a function $\mathcal{G}$ that maps the wavefront error map and star position to the observed focal plane image:

\begin{equation}
y_{i} = \mathcal{G}(\phi_{i}, p_{star}).
\end{equation}

In practice, we have access to an approximate estimate of the wavefront error map, denoted as $\hat{\phi}_{i}$, derived from the available wavefront sensing data. 
Our differentiable simulator $\mathcal{G}_{sim}$ takes this estimated wavefront error map and the star position as inputs, and generates a simulated focal plane image $\hat{y}_{i}$:

\begin{equation}
\hat{y}_{i} = \mathcal{G}_{sim}(\hat{\phi}_{i}, p_{star}).
\end{equation}

The simulation process in $\mathcal{G}_{sim}$ is implemented as a sequence of differentiable operations that model the propagation of light through the optical system. 
Starting with a plane wave representation of the incident light, we apply a series of transformations capturing the effects of the key optical elements in the coronagraphic system.

First, a phase shift is applied to the input wave to account for the position of the central star:

\begin{equation}
x^{(1)} = x \cdot e^{i p_{star}}.
\end{equation}

Next, the estimated wavefront error map is incorporated as an additional phase term:

\begin{equation}
x^{(2)} = x^{(1)} \cdot e^{i \hat{\phi}}.
\end{equation}

The wave is then propagated through the pupil plane optics, which include the entrance pupil function $P$ and the apodization function $A$:

\begin{equation}
x^{(3)} = A \cdot P \cdot x^{(2)}.
\end{equation}

The resulting wavefront is propagated to the focal plane using the Fourier transform operator $\mathcal{F}$, and the focal plane mask $B$ is applied:

\begin{equation}
x^{(4)} = B \cdot \mathcal{F}{x^{(3)}}.
\end{equation}

The masked wavefront is then propagated to the Lyot stop plane, where the Lyot stop function $C$ is applied:

\begin{equation}
x^{(5)} = C \cdot \mathcal{F}{x^{(4)}}.
\end{equation}

Finally, the wavefront is propagated to the science focal plane to obtain the simulated focal plane image:

\begin{equation}
\hat{y} = |\mathcal{F}{x^{(5)}}|^2.
\end{equation}


The optimization objective is to minimize the discrepancy between the simulated and observed focal plane images, given the current estimate of the wavefront error map. 
Formally, we seek to solve the following optimization problem:

\begin{equation}
\hat{\phi}_{i} = \operatorname*{argmin}_{\phi_{i}} \mathcal{L}(\mathcal{G}_{sim}(\phi_{i}, p_{star}), y_{i}),
\end{equation}

where $\mathcal{L}$ is a suitable distance metric, and we adopt the $L_1$ norm in our experiments. 
By leveraging the differentiability of $\mathcal{G}_{sim}$, we compute the gradients of the loss function with respect to the estimated wavefront error map $\hat{\phi}{i}$ and perform iterative gradient descent updates to refine the estimate. 
This optimization process encourages the estimated wavefront error map to better explain the observed images, improving the accuracy of the wavefront error estimates and the fidelity of the reconstructed stellar PSF.

Our approach integrates machine learning techniques with physics-based modeling to extract previously inaccessible information from the science camera observations. 
By leveraging differentiable programming, we efficiently invert the image formation process and infer critical wavefront error information that is not directly measured by the wavefront sensor. 
This enables the construction of accurate models of the stellar PSF, essential for effectively subtracting the starlight and revealing the faint exoplanet signals.


\subsection{Simulation Experiments}
To validate and demonstrate the potential of our proposed differentiable simulation approach for enhanced exoplanet imaging, we conducted a series of simulation experiments.
The primary objectives were to: (1) assess the effectiveness of using differentiable simulation to refine the wavefront error estimate and improve the accuracy of the estimated stellar PSF for starlight subtraction;
(2) evaluate the robustness of the method under variations in planet location and time-varying wavefront errors;
and (3) examine the progression of the wavefront error estimation and starlight subtraction over the course of the optimization process.

The simulator parameters were chosen to mimic typical scenarios in high-contrast imaging, with a contrast level range of $10^{-6}$ to $10^{-10}$ and varying levels of wavefront error. 
For each simulated scenario, we generated a ``ground truth'' wavefront error map $\phi_{i}$ and injected a planet signal at a specified location $p_{planet}$. 
The initial ``imperfect measurement'' of the wavefront error $\hat{\phi}_{i}$ was obtained by adding uniformly generated noise to the ground truth $\phi_{i}$, with noise levels ranging from 0.5\% to 10\% of the amplitude of ground truth error $\phi_{i}$.


The optimization process was performed using the Adam optimizer with a learning rate of $10^{-10}$ and a mean absolute error loss function.
We ran the optimization for 200 iterations for each simulated case.
Our implementation uses PyTorch, an automatic differentiation library, for efficient computation of gradients throughout the simulation pipeline.

Figure~\ref{fig:contrast_v_noise} demonstrates the effectiveness of our differentiable simulation approach in refining the stellar PSF estimate for improved starlight subtraction. 
Each row corresponds to a different contrast level between the star and planet, ranging from $10^{-6}$ to $10^{-10}$. The columns show the results for different levels of wavefront error noise, from 0.5\% to 10\%.
In each cell, the "Before" image shows the result of subtracting an inaccurate stellar PSF derived from the imperfect initial wavefront error estimate $\hat{\phi}_{i}$. 
The residual speckle noise dominates and obscures the planet signal. 
The "After" image shows the result after using our optimization approach to refine the wavefront error estimate. 
The refined stellar PSF subtraction effectively removes the speckles while preserving the planet signal. 
These results showcase the potential for differentiable simulation to significantly enhance the contrast and detectability of faint exoplanet signals.

\input{figures/fig_8}

In Figure~\ref{fig:varying_location}, we examine the robustness of our method to variations in the underlying planet location. 
For a fixed contrast level ($10^{-9}$) and wavefront error noise level (10\%), we simulated scenarios with the planet placed at different locations in the image. 
The results demonstrate that the differentiable simulation approach consistently leads to effective starlight subtraction and preserves the planet signal across the variations in planet location. 
This robustness is important, as the planet location is not known a priori in real observations.

Figure~\ref{fig:vid_sequence} illustrates the performance of our method in a scenario with time-varying wavefront errors, mimicking the case of having multiple observations of the same system at different epochs. 
We simulated a sequence of observations with slowly evolving wavefront errors by adding time-correlated random perturbations to the initial error map. 
We applied our optimization approach considering the loss over all simulated observations. 
The results show that, despite the presence of time-varying errors, the planet signal is consistently revealed after subtracting the refined stellar PSF in each frame. 
The residual speckle noise levels do vary across the observations, depending on the specific wavefront error realization, but the planet remains robustly detectable.

To provide insight into the progression of the wavefront error refinement process, Figure~\ref{fig:optim_progress} shows intermediate results during the optimization for a single simulated case (contrast $10^{-9}$, 10\% wavefront error noise).
The estimated wavefront error map $\hat{\phi}_{i}$ is iteratively improved using gradient descent over the loss function, starting from the initial imperfect measurement. 
At each step, the updated $\hat{\phi}_{i}$ is used to render a simulated image $\hat{y}_{i}$, which is compared to the observed image $y_{i}$ to compute the loss. 
As the optimization progresses, the rendered images increasingly resemble the observations, indicating that the refined wavefront error map is converging towards the true underlying map. 
Correspondingly, the starlight subtraction using the refined stellar PSF becomes more effective at removing speckles while revealing the planet.

The simulation experiments provide a comprehensive assessment of our differentiable simulation approach for enhanced exoplanet imaging. 
The results demonstrate the method's effectiveness in refining wavefront error estimates, improving starlight subtraction, and increasing the detectability of faint exoplanet signals under a range of realistic conditions. 
The robustness of the approach to variations in planet location and time-varying wavefront errors highlights its potential for real-world applications. 
By leveraging the power of differentiable simulations and gradient-based optimization, our method opens up new possibilities for pushing the limits of high-contrast imaging and enabling the discovery of exoplanets that were previously hidden beneath the glare of their host stars.

\subsection{Discussion}
The differentiable simulation approach introduced in this work represents a significant advancement in post-processing techniques for high-contrast exoplanet imaging.
Traditional post-processing pipelines, such as LOCI~\cite{Lafrenire2007ANA} and KLIP\cite{Soummer2012Detection} do not consider wavefront sensing data directly in their starlight subtraction process. 
This omission is inevitable due to the limitations in the accuracy and completeness of wavefront measurements, which prevent their effective integration into post-processing algorithms.

Our differentiable simulation framework represents significant advances at two levels. 
First, it makes the consideration of wavefront sensing data practical and effective in the post-processing pipeline. 
By establishing a differentiable connection between the wavefront error maps and the observed focal plane images, we can leverage the power of gradient-based optimization to refine our estimates of the true wavefront errors. 
This approach allows us to extract valuable information from the wavefront measurements that were previously difficult to incorporate into traditional post-processing methods.
Second, the differentiable simulation approach enables significant improvements in the actual performance of starlight subtraction and exoplanet detection. 
By iteratively updating the estimated wavefront error maps to minimize the discrepancy between the simulated and observed images, we progressively improve the accuracy of our wavefront error estimates and, consequently, the fidelity of the reconstructed stellar PSF. 
This refined estimation of the stellar PSF directly translates into more effective speckle noise suppression and enhanced contrast in the post-processed images.

As demonstrated in our experiments, by integrating wavefront sensing data and enabling the extraction of previously inaccessible information from focal plane observations, our framework pushes the boundaries of what is achievable in high-contrast imaging.
The differentiable simulation approach introduced in this work represents a paradigm shift in post-processing techniques for exoplanet imaging. 
By making wavefront sensing data consideration practical and enabling significant improvements in starlight subtraction performance, our framework opens up new possibilities for detecting and characterizing exoplanets that were previously hidden beneath the glare of their host stars





